It'll probably work out: improved list-decoding through random operations

In this work, we introduce a framework to study the effect of random operations on the combinatorial list-decodability of a code. The operations we consider correspond to row and column operations on the matrix obtained from the code by stacking the codewords together as columns. This captures many natural transformations on codes, such as puncturing, folding, and taking subcodes; we show that many such operations can improve the list-decoding properties of a code. There are two main points to this. First, our goal is to advance our (combinatorial) understanding of list-decodability, by understanding what structure (or lack thereof) is necessary to obtain it. Second, we use our more general results to obtain a few interesting corollaries for list decoding: (1) We show the existence of binary codes that are combinatorially list-decodable from $1/2-\epsilon$ fraction of errors with optimal rate $\Omega(\epsilon^2)$ that can be encoded in linear time. (2) We show that any code with $\Omega(1)$ relative distance, when randomly folded, is combinatorially list-decodable $1-\epsilon$ fraction of errors with high probability. This formalizes the intuition for why the folding operation has been successful in obtaining codes with optimal list decoding parameters; previously, all arguments used algebraic methods and worked only with specific codes. (3) We show that any code which is list-decodable with suboptimal list sizes has many subcodes which have near-optimal list sizes, while retaining the error correcting capabilities of the original code. This generalizes recent results where subspace evasive sets have been used to reduce list sizes of codes that achieve list decoding capacity.

==> general.tex <==
general stuff (stable boolean functions and etc) goes here.


==> general_col.tex <==
Our general result about column operations is based on the following version of Bernstein's inequality, which relies on the Orlicz norm $\| X\|_{\psi_1}$.  
\begin{definition}
For a random variable $Y \in \R$, define the $\psi_1$-norm by
%\[ \| Y \|_{\psi_1} = \inf\inset{ K \geq 0 \suchthat \EE \exp( |Y| / K ) \leq e }. \]
\begin{equation}\label{eq:moments}
 \| Y \|_{\psi_1} = \inf \inset{ K \geq 0 \suchthat \forall p > 0, \inparen{\EE |Y|^p}^{1/p} \leq Kp }.
\end{equation}
For a random vector $X \in \R^n$, we define
\[ \| X \|_{\psi_1} = \sup_{ y \in S^{n-1} } \| \ip{ y}{X} \|_{\psi_1}. \]
\end{definition}
\begin{remark} The $\psi_1$-norm is often defined by
\[ \| Y \|_{\psi_1} = \inf\inset{ K \geq 0 \suchthat \EE \exp( |Y| / K ) \leq e } \]
or by
\[ \|Y\|_{\psi_1} = \inf \inset{ K \geq 0 \suchthat \PR{ |Y| > t } \leq \exp \inparen{ 1 - \frac{t}{C\|X\|_{\psi_1} } }}. \]
\ar{In the above definition did you mean $t$ instead of $K$? And what is $X$?}
It is well-known (see~\cite{lt}) that these definitions are equivalent, up to constant factors.
\end{remark}
We will use a version of Bernstein's inequality that uses the $\psi_1$ norm~\cite{vw}. \TODO{cite Vandervaart and Wellner}
\begin{theorem}
Let $Y_1,Y_2,\ldots, Y_n$ be independent real-valued random variables with $\EE Y_i = 0$.  Let $\psi \geq \max_i \| Y_i \|_{\psi_1}$.
Then for all $t > 0$, 
\[ \PR{ \inabs{ \sum_i Y_i } > t } \leq 2 \exp \inparen{ \frac{ -t^2 }{ 4 \sum_{i \leq n} \| Y_i \|_{\psi_1}^2 + 2t\psi} }. \]
\end{theorem}

\TODO{$n_0$ and $n$ are used interchangeably. Need to use one notation.} \ar{I can do this once we decide on which one we choose. I guess $n_0$ would be more consistent with the rest of the paper?}
We have the following observation.
\begin{proposition}\label{prop:gencol}
The is a universal constant $C$ so that the following holds.
Let $f \sim \cD$ be a random column operation with independent codewords, so $f = (c_1,\ldots, c_N)$, where $c_i: \Sigma_0^{n_0 \times N_0} \to \Sigma^{n_0}$.  Suppose that for all $z$, $i$, 
\[ \| \agr( c_i(\cC_0) , z ) - \EE \agr( c_i( \cC_0), z )  \|_{\psi_1} \leq \psi. \]
Further, suppose that
\[ \frac{ \log_q(N) }{n_0} \leq \frac{C}{\log(q)} \min \left\{ \frac{ \eps  }{\psi }, n \inparen{ \frac{\eps }{\psi}}^2 \right\} \]
and that
\[ L \geq \max \inset{ \frac{ \psi }{\eps } , \frac{1}{n} \inparen{ \frac{\psi}{\eps } }^2 }. \]
\ar{I think there is a $\log{q}/C$ factor missing here-- for more see for comment in the proof.}
Suppose also that for all z and $\Lambda \subset [N]$ of size $L$, 
\[ \sum_{i \in \Lambda} \EE \agr( c_i(\cC_0), z) \leq nL\inparen{ 1/q + \eps/2 }. \]
Then with probability at least $1 - o(1)$, $\cC = f(\cC_0)$ is $(\rho, L)$-average-radius-list-decodable, for $\rho = 1 - 1/q - \eps$.
\end{proposition}
\begin{proof}
It suffices to show that with high probability, 
\[ \max_{\Lambda \subset [N], |\Lambda| = L} \max_{z \in \Sigma^n} \sum_{i \in \Lambda} \agr(z, c_i(\cC_0)) \leq nL\inparen{ \frac{1}{q} + \eps }. \]
For fixed $z$ and $\Lambda$, we write
\[ \sum_{i \in \Lambda} \agr( z, c_i(\cC_0) ) = \sum_{i \in \Lambda} \EE\agr( z, c_i(\cC_0) ) + \inparen{ \sum_{i \in \Lambda} \agr( z, c_i(\cC_0) ) - \EE \agr( z, c_i(\cC_0)) }.\]
The assumptions on the $\psi_1$ norm, along with Theorem \ref{thm:bernstein}, imply that that 
\[ \PR{  \sum_{i \in \Lambda} \agr( z, c_i(\cC_0) ) - \EE \agr( z, c_i(\cC_0)) > nL\eps/2 } \leq \inparen{ \frac{1}{ 2^n {N \choose L} }}^2. \]
In particular, a union bound over all $z$ and $\Lambda$, as well as our assumption on the expectation, completes the proof.
\ar{There are $q^n$ many $z$'s, so the $2^n$ should be $q^n$. This only increases the bound on $L$ by $\log{q}$, so no biggie.}
\end{proof}
Given this proposition, it is natural to ask how we might control the $\psi_1$-norm of $\agr(z,c_i(\cC_0))$.  For random subcodes, this reduces to understanding the list-decodability of $\cC_0$: indeed, suppose that each $c_i: \Sigma_0^{n_0 \times N_0} \to \Sigma_0^{n_0}$ is chosen independently from the set $\inset{ c(M) := M e_j \suchthat j \in [N_0] }$.  Then we have, for fixed $z$,
\begin{align*}
\PR{ \agr( c_i(M), z ) > t } = \frac{ | B( z, t ) \cap \cC_0 | }{ N_0 },
\end{align*}
which captures how the list size of $\cC_0$ grows with the radius $t$.  We can control this with the Johnson bound, and bounds on the weight distribution of  $\cC_0$.
\begin{lemma} \label{lem:weights}\TODO{ cite Gopalan-Klivans-Zuckerman'08 for this argument } 
Let $\cC_0 \subset \Sigma_0^{n_0}$ be any linear code of size $N_0$, and let $f= (c_1,\ldots, c_N)$ be the random column operation which selects a random subcode.  Let 
\[ A(\beta) = \frac{ \inabs{ \inset{ c \in \cC_0 \suchthat \agr(c,0) \geq \beta n_0 } }}{ N_0 } . \]
Fix $z \in \Sigma_0^{n_0}$.
Then with probability at least TBD,\ar{The statement below should be always true, right? I'm assuming this TBD is just copied over from some place else?}
\[ \PR{ \agr( c_i(\cC_0), z )  > \inparen{1/q + \gamma}n_0 } \lesssim \frac{ A( 1/q + \gamma ) }{\gamma^2}. \]
\ar{I'm pretty sure that the $A( 1/q + \gamma )$ term should be $A( 1/q + \gamma^2 )$. See below for more.}
\end{lemma}
\begin{proof} We borrow a proof from \cite{GKZ08}.  Let $\delta = 1 - 1/q - \gamma^2$, and let $\Lambda = B(z, 1 - 1/q - \gamma) \cap \cC_0$.  Let $S \subset \Lambda$ be a maximal $\delta$-separated set (so $d(c,c') \geq \delta$ for all $c,c' \in \Lambda$). Now $S$ forms a code of distance $\delta = 1 - 1/q - \gamma^2$, and it is contained in a ball of radius $1 - 1/q - \gamma$ about $z$, so by the $q$-ary Johnson bound, we have
\[ |S| \lesssim \frac{1}{\gamma^2}. \]
Now, for each $c \in \Lambda$, associate $c$ with the closest $c' \in S$ (breaking ties arbitrarily).  By linearity, at most $N_0 A(1/q + \gamma)$ codewords $c$ are associated with each $c' \in S$. \ar{This is where the bad typo is: note that we can only say that $d(c,c')\le 1-1/q-\gamma^2$ for $c'\in S$-- this means that the bound is $N_0 A(1/q + \gamma^2)$} Thus, we have
\[ \PR{ \agr(c_i(\cC_0), z) > \inparen{1/q + \gamma}n_0 } \leq |S|  A(1/q + \gamma)  \lesssim \frac{ A(1/q + \gamma) }{\gamma^2}, \]
as desired.
\end{proof}
To see the applicability of this, we consider Reed-Solomon codes. 
\begin{cor}[List-decodability of random subcodes of Reed-Solomon codes]
Let $\cC_0$ be a Reed-Solomon code over $\F_q$.  TBD.
\end{cor}
\begin{proof}
To apply Lemma \ref{lem:weights}, we recall the weight distribution of Reed-Solomon codes.  From Lemma 3.6 in~\cite{hartmanraz}, the number of polynomials of degree at most $d$ over $\F_q$ with exactly $k$ roots is bounded by
\[ \inabs{ \inset{ p \in \F_q[x] \suchthat \deg(p) \leq d, \text{ $p$ has $k$ roots } } } \leq q^{d+1} \inparen{ \frac{e + 1 }{k!} }. \]
Thus, the probability that a random polynomial (codeword) has $t$ roots is
\[ \PR{ \agr( c_i(\cC_0), 0 ) \geq t } \leq \sum_{k=t}^n \frac{ e + 1 }{k!} \lesssim \frac{ 1 }{ t! } \]
We apply Lemma \ref{lem:weights} to conclude that for all $z$,
\[ \PR{ \agr(c_i(\cC_0), z) \geq \inparen{1/q + \gamma}n_0 } \lesssim \frac{ 1}{(n(1/q + \gamma))!} \inparen{ \frac{1}{\gamma} }^2. \]
\ar{Propagating the change in Lemma~\ref{lem:weights} here, the factorial should be $(n(1/q + \gamma^2))!$.}
From this, we compute the $\psi_1$ norm of the mean-zero random variables
\[ Y_i: = \agr( c_i(\cC_0, z) ) - \EE \agr( c_i(\cC_0, z) ). \]
Notice first that $\EE \agr( c_i( \cC_0, z) ) = n/q$, and so the above reads
\begin{equation}\label{eq:tail}
 \PR{ |Y_i| \geq \gamma n } \lesssim \frac{ 1}{ (n(1/q + \gamma))! } \inparen{ \frac{1}{\gamma} }^2.
\end{equation}
\ar{Again factorial should be $(n(1/q + \gamma^2))!$.}
We can now compute the $\| Y_i \|_{\psi_1}$ by bounding the moments $\EE |Y_i|^p$.  We have
\begin{align*}
\EE |Y_i|^p &= \sum_{t=0}^{n(1 - 1/q)} \PR{ |Y_i|^p \geq t } \\
&\lesssim \int_{t=0}^{n(1 - 1/q)} \max \inset{ 1, \frac{ 1 }{ (t^{1/p} + n/q )! } \inparen{ \frac{n}{t^{1/p}} }^2 }\, dt \\ 
&\leq \int_{s=0}^{\infty} \max \inset{ 1 , \frac{1}{(s + n/q)!} \inparen{ \frac{n}{s} }^2 p s^{p-1} }\, ds 
\end{align*}
\ar{In the above calculation, the difference between $\gamma^2$ vs $\gamma$ seems to rear its ugly head. Two lines above, the term $t^{1/p}$ in the factorial should be $t^{2/p}/n$. In turn in the next line in the factorial $s$ should be replaced by $s^2/n$. This seems to be really bad for the rest of the calculations. In particular, I can make the subsequent calculations work only with $\tau$ something like $\sqrt{n}$, which is too much since it shows up in the rate (it also shows up in the list size but that is not a big deal.}
We will put the cut-off point at 
\[ \tau:= C \log(n), \]
for some constant $C$ to be determined in a moment.
\begin{align*}
\EE |Y_i|^p &\lesssim \int_{s=0}^{\tau } p s^{p-1} \,ds + \int_{s=\tau}^\infty \frac{1}{s!} \inparen{ \frac{n}{s} }^2 p s^{p-1}\, ds \\
&= \inparen{ \tau }^p + \int_{s = \tau}^\infty \frac{1}{s!} \inparen{ \frac{n}{s} }^2 p s^{p-1} \, ds \\
&\lesssim \tau^p + p n^2 \int_{s =\tau}^\infty \inparen{ \frac{e}{s} }^s  s^{p-3} \, ds \\
&\leq \tau^p + p n^2 \int_{s =\tau}^\infty \inparen{ \frac{e}{\tau} }^s  s^{p-3} \, ds.
\end{align*}
We may bound the integral (as long as $\tau \geq e^2$, which we will choose) by the incomplete gamma function
\[ \int_{s=\tau}^\infty e^{-s} s^{p-3}\,ds = \Gamma( p-2, \tau ) \leq e^{-\tau} (e\tau)^{p-2}. \]
Thus, 
\[ \frac{1}{p} \inparen{ \EE |Y_i|^p }^{1/p} \lesssim \tau +  p^{1/p - 1} n^{2/p} e^{-\tau} (e\tau)^{1 - 2/p}. \]
Thus, choosing $C \geq 3$ or so sufficiently large, we have
\[ \frac{1}{p} \inparen{ \EE |Y_i|^p }^{1/p} \lesssim \log(n) \]
for all $p$, and hence
\[ \| Y_i \|_{\psi_1 } \lesssim \log(n). \]
Now we plug into Proposition \ref{prop:gencol}, and we see that there is a choice of 
\[ L \gtrsim \frac{ \log(n) }{\eps} \]
and 
\[ R \leq \frac{ \eps }{\log(n) } \]
so that as long as
\[ \frac{ \log_q(N) }{n} \leq R, \]
then $\cC = f(\cC_0)$ is $(L, 1 - 1/q - \eps)$-average-radius list-decodable.
\TODO{ the expectation (we just did the deviation) -- that will give us the correct $q\eps^2$ dependence as well. }

\begin{comment}
We bound the integral in two cases.  First, if $p \leq \tau/2$, then the term $(e/\tau)^s$ dominates the term $s^{p-3}$; more precisely, we have
\[ \int_{\tau}^\infty (e/s)^s s^{p-3} \leq \int_{\tau}^\infty e^s s^{-s/2 - 3} \leq \int_{\tau}^\infty e^{-s} = e^{-\tau}. \]
In this case, we have
\[ \EE |Y_i|^p \lesssim \tau^p + pn^2e^{-\tau}. \]
Thus, if we set $C \geq 2$, we have $\EE |Y_i|^p \lesssim \tau^p + p$, and
\[ \frac{1}{p} \inparen{ \EE |Y_i|^p }^{1/p} \lesssim \tau + \frac{1}{p}  \lesssim \tau. \]
On the other hand, if $p \geq \tau/2$, then the integral is about $(p-2)!$. \TODO{actually work out the gamma function.  This should not be so bad.  It should definitely work. }

\begin{align*}
 \int \inparen{ \frac{1}{\tau} }^{-s} s^{p-3}\,ds &= \ln^{2-p}(\tau) \Gamma( p-2 , \tau \ln(\tau)) \leq e^{-\tau} (e\tau)^{p-2} \\
&\leq \ln^{2-p}(\tau) \begin{cases} e^{-\tau \ln(\tau) } & \tau \geq 100p \\
(p-2)! & \text{ any } \tau,p \end{cases} \\
\end{align*}
Then for $4 \leq p \leq \log(n)$ or so, we have 
\[ \EE |Y_i|^p \lesssim \tau^p + pn^2 \ln^{2-p}(\tau) \frac{1}{\tau^\tau} . \]
Thus, setting $C=e$, 
\[ \frac{1}{p} \inparen{ \EE|Y_i|^p }^{1/p} \lesssim 
\begin{cases} \inparen{ e\log(n) }^p + p & p \leq 3 \\
 e\log(n) + n^{2/p} \inparen{ \log \inparen{e \log(n)}}^{2/p - 1} (p-2)^{-2/p} &p > 3 \end{cases} \]
This is maximized when $p=4$
Thus, we have, for all $i$, 
\[ \left\| Y_i \right\|_{\psi_1} \lesssim \sqrt{ \frac{n}{\log\log(n)} }. \]
Now, we may plug this bound into Proposition \ref{prop:gencol}.
\TODO{Oops, I need a different Bernstein's inequality.  I think I need the one where the Gaussian term is controlled by $\sigma_i$.  For this definition, I need $\PR{ X \geq t } \leq \exp(-t^2/\sigma^2)$ when $t < \sigma^2/\|X\|_{\psi_1}$, which I think I get from normal Bernstein.  Def would be
\[ \ln( M_X(\lambda) ) \leq \lambda^2 \sigma^2/2 \]
for all $|\lambda| \leq 1/b$  (then it's $(\sigma,b)$-subexponential, and we get the right bound).}
\end{comment}
\end{proof}


==> useful.tex <==
In this section, we give several possibilities for the distribution $\cD$ of Theorem \ref{thm:mainthm}, and 
compute the corresponding parameter $\cE$.   This will give a list of random operations that one can do to codes which will maintain the
list-decoding radius.

\subsection{Random alphabet reduction}
Suppose that $\cC_0 \subset \Sigma_0^n$ is a code over a large alphabet, and we wish to obtain a code over a smaller alphabet, $\Sigma$.  One option is to concatenate $\cC_0$ with a code over $\Sigma$; however, this will cause the block length to increase.
Another option is to map each symbol $c_j \in \Sigma_0$ to $\Sigma$ via, say, some hash function.  To that end, we consider the following set-up.

Let $\mathcal{H}$ be a family of hash functions $h: \Sigma_0 \to \Sigma$ with collision probability $p$: that is, if $h \in \mathcal{H}$ is chosen uniformly at random, then for any $c \neq c' \in \cC_0$,
\[ \PR{ h(c) = h(c') } = p. \]
For example, if $\mathcal{H}$ is a pairwise independent family, then $p = 1/|\Sigma|$.
In this case, we may use the average-radius Johnson bounds in Theorem \ref{thm:jb} (using whichever is appropriate for the size of $\Sigma$), along with Theorem \ref{thm:mainthm}, to obtain the following statement.

\begin{theorem}\label{thm:hashes}
Suppose that $\mathcal{H}$ is as above, and let $\cC_0$ be any code with distance $\delta$.  Then \TODO{fill in what you get for big $q$ and for small $q$}
\end{theorem}



